From Black-Scholes to Online Learning: Dynamic Hedging under Adversarial Environments

We consider a non-stochastic online learning approach to price financial options by modeling the market dynamic as a repeated game between the nature (adversary) and the investor. We demonstrate that such framework yields analogous structure as the Black-Scholes model, the widely popular option pricing model in stochastic finance, for both European and American options with convex payoffs. In the case of non-convex options, we construct approximate pricing algorithms, and demonstrate that their efficiency can be analyzed through the introduction of an artificial probability measure, in parallel to the so-called risk-neutral measure in the finance literature, even though our framework is completely adversarial. Continuous-time convergence results and extensions to incorporate price jumps are also presented.

==> amodel.tex <==

{\color{blue} \Znote{we need to take care of this crap}
\section{Model comparison}\label{sec:modelcomp}
We note that the model studied in this paper is closely related to the one studied in~\cite{AFW12}.
 There, they impose a round-wise second moment constraint on the adversary. When the payoff function is convex, both constraints are equivalent algorithmically (see Section~\ref{sec:convexmultiround}).  When the payoff function is non-convex, the adversary may want to
impose sparse jumps in its optimal strategy in~\cite{AFW12}'s model (and thus violating our uncertainty set constraints) but then second moment would not be
a natural constraint for jumps (see discussions in~\cite{cont2012financial}). Section~\ref{sec:jump} discusses how we incorporate price jumps in our model.
}

==> apropdual.tex <==
\subsection{Proof of Proposition~\ref{prop:dual}}\label{asec:dual}
We now generalize the proof for Proposition~\ref{prop:dual} to general uncertainty set case, with slightly more function space technicalities. For general uncertainty set $\mathcal U$, we can generalize (\ref{eqn:primal}) as:
\begin{equation}
\begin{array}{ll}
\mbox{minimize}&p\\
\text{subject to}&p+r\Delta\geq g(S_0(1+r)) \text{\ \ for $r \in \mathcal U$}
\end{array} \label{eqn:cprimal}
\end{equation}
Next, note that the dual cone of $\mathcal C^+(\mathcal U)$, the set of non-negative continuous functions on $\mathcal U$, is $P^+(\mathcal U)$, the set of positive measures on $\mathcal U$. Since $g$ is assumed to be continuous, the Lagrangian of \eqref{eqn:cprimal} is
$$L(p,\Delta,w)=p+\int_{\mathcal U}(g(S_0(1+r))-r\Delta-p)dw(r)$$
where $w(\cdot)\in\mathcal P^+(\mathcal U)$ (see~\cite{luenberger1997optimization}). The dual function is defined as
\begin{align}
\ell(w)&=\inf_{p,\Delta}\left\{p+\int_{\mathcal U}(g(S_0(1+r))-r\Delta-p)dw(r)\right\}\notag\\
&=\inf_{p,\Delta}\left\{\int_{\mathcal U}g(S_0(1+r))dw(r)+(1-w(\mathcal U))p+\int_{\mathcal U}rdw(r)\Delta\right\} \label{eqn:dual function}
\end{align}
Suppose $w(\cdot)$ does not satisfy either $w(\mathcal U)=1$ or $\int_{\mathcal U}rdw(r)=0$, then one can always find $p$ or $\Delta$ that gives arbitrarily large objective value in \eqref{eqn:dual function}. Hence the dual problem $\max_{w\in\mathcal{P}^+(\mathcal U)}\ell(w)$ can be written as
%Let $w(r) \geq 0$ be a function in $\mathcal U$. The Lagrange of (\ref{eqn:cprimal}) is
%$$L(w, p, \Delta) = \int_{-\uzeta}^{\ozeta}w(r)\left\{-p - Sr\Delta + g(S(1+r)\right\}dr.$$
%So the dual function $\ell(\cdot)$ is
%\begin{eqnarray*}
%\ell(w) & = & \inf_{p^*, \Delta^*}\int_{-\uzeta}^{\ozeta}w(r)\left\{-p - Sr\Delta + g(S(1+r)\right\}dr \\
%& = & \inf_{p^*, \Delta^*}\left\{\int_{-\uzeta}^{\ozeta}w(r)g(S(1+r))dr - \left(\int_{-\uzeta}^{\ozeta}w(r)dr - 1\right)p^* - \left(\int_{-\uzeta}^{\ozeta}rw(r)dr\right)S\Delta^*\right\}
%\end{eqnarray*}
%The infimum of a linear function is $-\infty$ except in the special case when it is identically zero. So we can express the dual function as
%
%\begin{equation}
%\begin{array}{ll}
%\mbox{maximize}&\int_{-\uzeta}^{\ozeta}w(r)g(S(1+r_i))dr\\
%\text{subject to}&\int_{-\uzeta}^{\ozeta}w(r)dr=1\\
%&\int_{-\uzeta}^{\ozeta}w(r)rdr=0\\
%&w(r)\geq0\text{\ \ for $r\in\mathcal U$}
%\end{array} \label{eqn:cdual}
%\end{equation}
\begin{equation}
\begin{array}{ll}
\mbox{maximize}&\int_{\mathcal U}g(S_0(1+r))dw(r)\\
\text{subject to}&\int_{\mathcal U}rdw(r)=0\\
&w(\mathcal U)=1\\
&w\in\mathcal{P}^+(\mathcal U)
\end{array} \label{eqn:cdual}
\end{equation}

Finally, it is easy to see that the constraint set in \eqref{eqn:cprimal} has non-empty interior (by picking large enough $p$ for example). Hence strong duality holds and the dual optimal value in (\ref{eqn:cdual}) equals the primal counterpart (see \eg Chapter 8 in~\cite{luenberger1997optimization}). By identifying $w$ as a probability measure on $\mathcal U$, we conclude that \eqref{eqn:cdual} is the same as \eqref{eqn:char}. This completes our proof.


==> miscellaneous.tex <==

\iffalse
\begin{proof}
To illustrate the key idea in our analysis, let us start with analyzing a ``discrete" version of the problem, \ie let $\mathcal U = \{r_1, r_2, ..., r_n\}$ be a discrete set on $\mathbb{R}$. We can write $\min_{\Delta}\max_{R \in \mathcal U}g(S_0(1+R)) - R \Delta$ as the following linear program (LP):
{{
\begin{equation}
\begin{array}{ll}
\mbox{min}&p\\
\text{s.t.}&g(S_0(1+r_i))-r_i\Delta\leq p \text{\ \ for $i\in[n]$}
\end{array}
\mbox{ $\equiv$ }
\begin{array}{ll}
\mbox{min}&p\\
\text{s.t.}&p+r_i\Delta\geq g(S_0(1+r_i))\text{\ \ for $i\in[n],$}
\end{array} \label{eqn:primal}
%\label{eq`n:primal interim}
\end{equation}}}
where the decision variables are $p$ and $\Delta$. The formulations in \eqref{eqn:primal} follow
simply by the definition of minimax problem, with the optimal $p$ representing the option price's upper bound. Now we invoke the standard primal-dual theorem for LP on \eqref{eqn:primal} and obtain the following equivalent LP in dual form:

%
%The constraints simply read as follow: regardless the choice of $r_i$ by the adversary, the difference between the option's payoff and the investor's return is at most $p$. Thus, the optimal $p^*$ in (\ref{eqn:primal}) is the upper bound for the option's price. Now we invoke a standard primal-dual theorem for linear program on \eqref{eqn:primal} and obtain the following equivalent linear program in dual form:
{\small
\begin{equation}
\begin{array}{ll}
\mbox{maximize}&\sum_{i\in[n]}w_ig(S_0(1+r_i))\\
\text{subject to}&\sum_{i\in[n]}w_i=1\\
&\sum_{i\in[n]}w_ir_i=0\\
&w_i\geq0\text{\ \ for $i\in[n]$}
\end{array} \label{dual}
\end{equation}
}
Here $w_i$'s are the decision variables. Observe that $\{w_i\}_{i \in [n]}$ can be interpreted as a probability distribution on the uncertainty set $\mathcal U$ since $\sum w_i=1$. Call this distribution $P_f$. This is a risk-neutral probability distribution since the expected return $\E_{P_f}[R]=\sum w_ir_i=0$. Moreover, note that the objective function under this probability interpretation can be rewritten as $\sum_{i\in[n]}w_ig(S(1+r_i)) = \E_{R\leftarrow P_f}[g(S(1+R))]$. We thus have proved (\ref{eqn:char}).
The generalized argument appears in Appendix~\ref{asec:dual}.

\end{proof}
\fi



\section{Generalizations.}\label{sec:genshort}
This section generalizes our results in three ways: 1. We show that our minimax upper bound of the option price, with possibly non-convex payoff, converges to the price based on a controlled diffusion process when the uncertainty sets are appropriately scaled. 2. We extend our dual characterization, convergence, and algorithmic results to American-type options.   3. We extend our model to cover ``shocks" in the financial market. In the stochastic framework, these are typically modeled as Poisson arrivals of jumps on top of a continuous geometric Brownian motion on the asset price. We will adopt our adversary framework to incorporate these price jumps.

\myparab{Convergence to controlled diffusion process} (see Appendix~\ref{sec:control} for details).
To facilitate discussion, here we let the time steps be $0,\delta,2\delta,\ldots,T$ (for simplicity let $T$ be a multiple of $\delta$), and thus $\tau = \frac{T}{\delta}$. Let $\mathcal{U}^\delta=[-\uzeta^\delta,\ozeta^\delta]$, where $-\uzeta^\delta\triangleq-\uzeta\sqrt{\delta}$ and $\ozeta^{\delta} \triangleq \ozeta\sqrt{\delta}$. Recall that we write $S(t)$ as the continuous-time price of the underlying asset at time $t$, with $S(0) = S_0$ (this process is decided by nature). We have the following theorem:
%We also denote $g_i^\delta(x)$ as the value function of the upper bound's dynamic program at the $i$-th round evaluated as $x$. Our goal is to show that $\lim_{\delta\to0}g_0^\delta(x)$ exists and is equal to the expected payoff of a controlled diffusion model. We have the following theorem:

\begin{theorem}\label{thm:continuous}
Let $g$ be a Lipschitz continuous payoff function. As $\delta\to0$, the upper bound of the option price defined by $
\min_{\Delta_1,\Delta_2,\ldots,\Delta_{\tau}}\max_{R_1^\delta,\ldots,R_{\tau}^\delta\in\mathcal{U}^\delta}g\left(S_0\prod_{i=1}^{\tau}(1+R_i^\delta)\right)-\sum_{i=1}^{\tau}\Delta_iR_i^\delta$
converges to %$\max_\xi \E[g(S(T))]$.
\begin{equation}
G(0,S_0):=\max_\xi \E[g(S(T))]. \label{value continuous}
\end{equation}
Here $S(t)$ follows the dynamic
$dS(t)=\sigma(u)S(t)dw(t)$, where $w(t)$ is a standard Brownian motion, $\sigma(u)=u$ is the controlled volatility, and $\xi=\{u(t),0\leq t\leq T:u(t)\in U\}$ is an adapted control sequence. The domain of control $U=[0,\underline{\zeta}\overline{\zeta}]$.
\end{theorem}
Intuitively, this theorem asserts that the continuous-time limit of the option price's upper bound for non-convex payoff is Gaussian in nature, similar to the case of convex payoff and Black-Scholes model. The crucial difference with those cases, however, is that nature now has the additional power to choose (to reduce) the volatility at any point of time, and this is only helpful to nature in the case of non-convex payoff. Since we know from Section~\ref{sec:non-convex} that in the discrete-time setting with non-convex payoff, the nature does not necessarily choose the extremal point in the uncertainty set, it is not surprising that there is reduction in volatility at certain points of time in the continuous-time counterpart.

\myparab{American Options} (see Appenix~\ref{sec:american} for details)
We generalize our results to American-type option. We will give a dual characterization using risk-neutral measure, and from there we will obtain convergence and algorithmic results similar to European-type options. As before, let us first consider the single-round game.

%we shall first give a characterization on optimal solution from the dual program. This characterization suffices to show that the multinomial tree approximation will give a good approximation. We then analyze the special case when the payoff function $g(\cdot)$ is convex. We shall show that in this case the interval market model also converges to the Black-Scholes-Merton model. Finally, we briefly discuss a model with a more powerful adversary, \ie the investor is allowed to trade at discrete time intervals while the adversary can exercise the American option at any moment. We shall show that under mild condition, our results also extend to this model.

%\myparab{Single-round American option game.}
%We start with analyzing the one-round equilibrium in our interval market model.

In the single round game, the upper bound of an American option can be expressed as:\\
$
\min_{\Delta}\max_{\substack{\theta\in \{0, 1\}\\R \in \mathcal U}}\left((g(S_0(1+R))-R\Delta)(1-\theta) + g(S_0)\theta\right)$ (*), where $\theta$ is the decision made by the adversary in exercising the option prematurely: $\theta=1$ if early exercise is prompted, otherwise $\theta=0$. We remark that it is the adversary, not the trader, to have the right to exercise early in upper bound evaluation. It is because the upper bound comes from a short-option argument (see Section~\ref{sec:model}) that endows nature as the holder of the option and hence the early exercise right. Our first result shows that the above optimization formulation (*) equals to
$\max_{\theta}\min_{\Delta}\Phi(\Delta,\theta)$ (see the full version of the paper). We also have similar results for lower bounds.

Using the results for single round game, we can analyze the general case. Specifically, we have:
\begin{lemma}Consider a $\tau$-round American option hedging game with convex payoff function $g(\cdot)$ and uniform uncertainty set $\mathcal U = [-\uzeta, \ozeta]$. The option price's upper bound is the same as the $\tau$-round binomial tree model. Moreover, if $U$ scales appropriately, the upper bound converges to the Black-Scholes price.
\end{lemma}

Finally, let us briefly comment on the algorithm for American options.
The algorithm for computing American options over binomial trees can be found in, for example,~\cite{hull2009options}, which implies early exercise for put option but not call option.
%Here, the reader only needs to think the binomial tree model as a special case for of the interval market model except that the uncertainty set there is two singular points $ \{-\uzeta, \ozeta\}$.
For non-convex payoff in upper bound calculation, or any payoff in lower bound calculation, the reduction to binomial tree does not necessarily hold. One can resort to our multinomial tree algorithm presented in Section~\ref{sec:non-convex} to approximate.
\begin{corollary} Let $\delta$ be an arbitrary constant. Consider using the multinomial tree approximation algorithm to find the American option's upper bound. When $\epsilon = c \delta^2/(L^2\tau^2)$ for some constant $c$, the algorithm gives an $\hat g_0(S_0)$ such that $g_0(S_0) - \delta S_0 \leq \hat g_0(S_0) \leq g_0(S_0)$.
\end{corollary}

We remark that one arguably unsatisfying feature in our model for the upper bound of American options is that the nature can only exercise the option at discrete rounds, \ie at the times when the trader can execute trade decisions. Appendix~\ref{sec:american} discusses how this issue can be addressed.

\myparab{Integration with jumps} (see Appendix~\ref{sec:jump} for details)
As discussed above, allowing jumps is a natural way to model ``shocks'' in the movement of the stock price.
There can be various ways to model when and how much the adversary can control the price to jump. We analyze two natural examples that can be extended from our framework. Here, we sketch the formulation for one of them. The other example and the algorithms for both of them are in Appendix~\ref{sec:jump}.

\mypara{Example 1.  The random jump model.}
This model assumes a convex payoff function and that the nature performs a jump with a prefixed small probability $q$ at each step. If a jump occurs, the nature moves according to a return $Y$ that is random (whose distribution is given). Otherwise, with $1-q$ probability, the nature will have freedom to choose its path inside the uncertainty set $\mathcal{U}$. We also assume $q$ is sufficiently small (see the full version of the paper). %, \ie $-pE_Y[Y]-\overline{\zeta}(1-p)\geq0$ and $(1-p)\underline{\zeta}+pE_Y[Y]\geq0$ (CHECK)




==> missingcal.tex <==
\section{Missing calculation}\label{sec:missing}
\myparab{Proof of (\ref{eqn:prob1})}
\begin{align}
\frac{\hrtwo}{\hrtwo-\hrone}&=\frac{\rtwo}{\rtwo-\rone}+\frac{\hrone\rtwo-\hrtwo\rone}{(\hrtwo-\hrone)(\rtwo-\rone)} \notag\\
&=\frac{\rtwo}{\rtwo-\rone}+\frac{\rtwo(\hrone-\rone)-\rone(\hrtwo-\rtwo)}{(\hrtwo-\hrone)(\rtwo-\rone)} \notag\\
&\geq\frac{\rtwo}{\rtwo-\rone}-\frac{\rtwo\epsilon}{(\hrtwo-\hrone)(\rtwo-\rone)}\text{\ \ (since $-\hrone(\hrtwo-\rtwo)\geq0$ and $|\hrone-\rone|<\epsilon$)} \notag\\
&\geq\frac{\rtwo}{\rtwo-\rone}-\frac{\rtwo\epsilon}{(\rtwo-\rone)^2}\text{\ \ (by construction we have $\hrtwo-\hrone\geq\rtwo-\rone$)} \notag\\
&\geq\frac{\rtwo}{\rtwo-\rone}\left(1-\frac{\epsilon}{\eta}\right) \notag%\label{eqn:prob1}.
\end{align}

